End-to-End Orchestration of NextG Media Services over the Distributed Compute Continuum

NextG (5G and beyond) networks, through the increasing integration of cloud/edge computing technologies, are becoming highly distributed compute platforms ideally suited to host emerging resource-intensive and latency-sensitive applications (e.g., industrial automation, extended reality, distributed AI). The end-to-end orchestration of such demanding applications, which involves function/data placement, flow routing, and joint communication/computation/storage resource allocation, requires new models and algorithms able to capture: (i) their disaggregated microservice-based architecture, (ii) their complex processing graph structures, including multiple-input multiple-output processing stages, and (iii) the opportunities for efficiently sharing and replicating data streams that may be useful for multiple functions and/or end users. To this end, we first identify the technical gaps in existing literature that prevent efficiently addressing the optimal orchestration of emerging applications described by information-aware directed acyclic graphs (DAGs). We then leverage the recently proposed Cloud Network Flow optimization framework and a novel functionally-equivalent DAG-to-Forest graph transformation procedure to design IDAGO (Information-Aware DAG Orchestration), a polynomial-time multi-criteria approximation algorithm for the optimal orchestration of NextG media services over NextG compute-integrated networks.

==> notation_table_OLD.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{|c|l|}
    \hline
    Notation & Definition \\
    \hline
    % NETWORK
    $\mathcal G$ & NextG cloud-integrated network\\
    $\mathcal V$ & Network nodes\\
    $\mathcal E$ & Network links\\
    $\mathcal G^a$ & Cloud-augmented graph\\
    $\mathcal V^a$ & Augmented network nodes\\
    $\mathcal E^a$ & Augmented network links\\
    
    $\mathcal V^p$ & Computation nodes\\
    $\mathcal V^s$ & Source nodes\\
    $\mathcal V^d$ & Destination nodes\\

    $\mathcal E^p$ & Computation links\\
    $\mathcal E^s$ & Source links\\
    $\mathcal E^d$ & Destination links\\

    $c_{uv}$ & Capacity at link $(u,v)$\\
    $w_{uv}$ & Cost at link $(u,v)$\\

    % SERVICE
    $\mathcal R$ & NextG information-aware service DAG set of service\\
    $\mathcal I$ & Service functions\\
    $\mathcal K$ & Commodities\\
    
    $\mathcal K^s$ & Source commodities (commodities produced by a source function)\\
    $\mathcal K^d$ & Destination commodities (commodities produced by a source function)\\
    $\mathcal K^p$ & Processing commodities (commodities produced by a processing function)\\

    $\mathcal I^s$ & Source functions\\
    $\mathcal I^d$ & Destination functions\\
    $\mathcal I^p$ & Computation functions\\

    $R^k_{uv}$ & Size or rate of commodity $k \in \mathcal K$ when it goes over link $(u,v) \in \mathcal E^a$\\
    
    $\mathcal X(k)$ & Set of input commodities required to produce commodity $k \in \mathcal K$\\
    
    $s^{\mathcal K}(k)$ & The node hosting the function producing source commodity $k \in \mathcal K^s$\\
    $d^{\mathcal K}(k)$ & The node hosting the function producing destination commodity $k \in \mathcal K^d$\\
    $s^{\mathcal I}(i)$ & The node hosting the function hosting source function $i \in \mathcal I^s$\\
    $d^{\mathcal I}(i)$ & The node hosting the function hosting destination function $i \in \mathcal I^d$\\

    $\mathcal O$ & Set of information object\\
    $g:\mathcal K \rightarrow O$ & information mapping function\\

    % Latency
    $l^k$ & Local latency\\
    $l^k_{uv}$ & latency to transmit or process a unit of commodity $k$ over link $(u,v)$\\
    $l^k_T$ & Aggregate latency (service latency accumulated until the consumption of commodity k) \\
    $L^k$ & Maximum allowed service latency\\

    $f_{uv}^k$ & Virtual Commodity Flow\\
    $\mu_{uv}^o$ & Actual information object flow\\
    $\mu_{uv}$ & Actual information flow\\

    $\mathcal R^T$ & Service graph after DAG-to-Forest transformation\\
    $\mathcal I^T$ & Service graph function after DAG-to-Forest transformation\\
    $\mathcal K^T$ & Service graph commodities after DAG-to-Forest transformation\\


    $g_T:\mathcal K^T \rightarrow O$ & \red{Information mapping function}\\

    $\mathcal R^{T,\phi}$ & $\phi-th$ connected component of transformed service graph $\mathcal R^T$\\

    $\mathcal I^{d,T}$ & Set of destination function of $\mathcal R^T$\\
    $\mathcal I^{d,T,\phi}$ & Set of destination function of $\mathcal R^{T,\phi}$\\

    $\mathcal V^{p,\mathcal K}(k)$ & Set of nodes that can process commodity $k \in \mathcal K$\\ 
    $\mathcal V^{p,\mathcal I}(i)$ & Set of nodes that can process function $i \in \mathcal I$\\

    $\map^{\mathcal I}$ & Function mapping\\
    $\map^{\mathcal K}$ & Commodity mapping\\

    $\Emb^\phi$ & \red{Embedding}\\
    $\Emb$ & \red{Embedding}\\
    $p^\phi$ & Associated probability\\
    
    $\mathcal D^\phi$ & Decomposition\\
    $\mathcal D$ & Decomposition\\

    $\flD$ & Commodity flow Decomposition \\
    $\muD$ & Information flow Decomposition \\
    
    $\flR$ & Random commodity flow \\
    $\muR$ & Random information flow \\
    $\fLP^k_{u,v}$ & Commodity flow solution to the LP relaxation of MILP\\

    $f^{\phi}_{\rightarrow{d}}$ & Total commodity flow consumed by the single destination function of $\mathcal R^{T,\phi}$\\

    $\Delta_\alpha$ & \\
    $\delta_\alpha$ & \\
    $\Delta_\beta$ & \\
    $\delta_\beta$ & \\
    $y_{uv}$ & Number of resoucre blocks allocated\\
    $c^b_{uv}$ & Capacity of each block \\
    $c^T_{uv}$ & Total number of blocks assignable over link $(u,v)$\\
        
    \hline
    \end{tabular}
    \caption{Table of Notation}
    \label{tab:notations}
\end{table*}


==> notation_table_short_OLD.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{|p{1.7in}|p{5in}|}
    \hline
    Notation & Description \\
    \hline
    % NETWORK
    $\mathcal G = (\mathcal V, \mathcal E)$; $\mathcal G^a = (\mathcal V^a, \mathcal E^a)$ & Network graph, nodes, and links; Cloud-augmented graph, nodes, and links\\

    %$\mathcal G^a = (\mathcal V^a, \mathcal E^a)$ & Cloud-augmented graph; Augmented network nodes; Augmented network links.\\
    
    $\mathcal V^p; \mathcal V^s; \mathcal V^d$ & Computation nodes; Source nodes; Destination nodes.\\

    $\mathcal E^c; \mathcal E^p; \mathcal E^s; \mathcal E^d$ & Communication links; Computation links; Source links; Destination links.\\

    $\mathcal E^{p-}; \mathcal E^{p+}$ & Computation in links (storage resources); Computation out links (processing resources).\\

    $\mathcal N^{-}(u); \mathcal N^{+}(u)$ & Incoming and outgoing neighbors of node $u\in\mathcal V^a$.\\

    $c_{uv}; w_{uv}$ & Capacity and cost at link $(u,v)$.\\
    
    % SERVICE
    $\mathcal R = (\mathcal I, \mathcal K)$ & Information-aware service (or service collection) graph, functions, and commodities \\
    
    $\mathcal K^s; \mathcal K^d; \mathcal K^p$ & Source commodities; Destination commodities; Processing commodities (i.e., produced by a processing function)\\

    % $\mathcal K^p$ & The set of commodities that are produced by a processing function.\\

        
     $\mathcal X(k)$ & Set of input commodities required to produce commodity $k$.\\

     
    $s^{\mathcal K}(k); d^{\mathcal K}(k)$ & Source node hosting the function producing commodity $k \in \mathcal K^s$; Destination node hosting the function consuming commodity $k \in \mathcal K^d$.\\
    
    % $d^{\mathcal K}(k)$ & The node hosting the function producing destination commodity $k \in \mathcal K^d$.\\

    $\mathcal I^s; \mathcal I^d; \mathcal I^p$ & Source functions; Destination functions; Computation functions.\\
        
    $s^{\mathcal I}(i); d^{\mathcal I}(i)$ & Node hosting source function $i \in \mathcal I^s$; Node hosting destination function $i \in \mathcal I^d$.\\


    % $d^{\mathcal I}(i)$ & The node hosting the function hosting destination function $i \in \mathcal I^d$\\

    $\mathcal V^{p,\mathcal I}(i)\equiv\mathcal V^{p,\mathcal K}(k)$ & Computation nodes that can host function $i$ and hence produce commodity $k$.\\

    $R^k_{uv}$ & Size or rate of commodity $k \in \mathcal K$ when it goes over link $(u,v) \in \mathcal E^a$.\\


    $\mathcal O$; $g:\mathcal K \rightarrow O$ & Set of information objects; Information mapping function.\\

    $f_{uv}^k; \mu_{uv}^o; \mu_{uv}$ & Virtual commodity flow,  actual information object flow, and actual information flow variables of MILP \eqref{eq:ilp}.\\    
    % $f_{uv}^k$ & Virtual Commodity Flow\\
    % $\mu_{uv}^o$ & Actual information object flow\\
    % $\mu_{uv}$ & Actual information flow\\

    % Latency
    $l^k_{uv}; l^k; l^k_T; L^k$ & Latency to transmit or process a unit of commodity $k$ over link $(u,v)$; Local latency of commodity $k$; Cumulative latency of commodity $k$; Maximum service latency associated with destination commodity $k$.\\
    
    % $l^k$ & Local latency\\
    % $l^k_{uv}$ & latency to transmit or process a unit of commodity $k$ over link $(u,v)$\\
    % $l^k_T$ & Cumulative latency (service latency accumulated until the consumption of commodity k) \\
    % $L^k$ & Maximum allowed service latency\\

    $\mathcal R^T = (\mathcal I^T, \mathcal K^T)$ & Forest graph after DAG-to-Forest transformation procedure.\\
    % $\mathcal R^T$ & Service graph after DAG-to-Forest transformation\\
    % $\mathcal I^T$ & Service graph function after DAG-to-Forest transformation\\
    % $\mathcal K^T$ & Service graph commodities after DAG-to-Forest transformation\\
    $\mathcal R^{T,\phi}$ & $\phi-th$ connected component (tree) of transformed service graph (forest) $\mathcal R^T$.\\

    $g_T:\mathcal K^T \rightarrow O$ & Information mapping function for transformed service graph $\mathcal R^T$.\\

    $M=|\mathcal K^d|$ & Number of connected components or service trees in transformed service graph $\mathcal R^T$.\\

    % ALGORITHM
    $\fLP^k_{uv}; \muLP^o_{uv}; \muLP_{uv}$ & Commodity flow, information object flow, and information flow variables of LP relaxation of MILP \eqref{eq:ilp}. \\

    $\fLP^{\phi}_{\rightarrow{d}}$ & Total commodity flow consumed by the single destination function of $\mathcal R^{T,\phi}$ throughout the Decomposition step of \alg.\\

    $\Emb^{\phi}_{n} = (m_n^{\phi,\mathcal I}, m_n^{\phi,\mathcal K)}$ & Valid Embedding, including function mapping and commodity mapping of service tree $\phi$ computed at iteration $n$ of the Decomposition step of \alg.\\

    $\miD^{\phi}= \left  \{ (\Emb^{\phi}_{1}, p^\phi_1) \ldots  (\Emb^{\phi}_{N_\phi}, p^\phi_{N_\phi}) \right \}$ & Decomposition of a service component, composed of a set of valid embeddings and associated probability.\\

    $N_\phi$ & Number of embeddings associated with service tree $\phi$.\\

    $\flD^k_{uv}; \muD^o_{uv}; \muD_{uv}$ & Commodity flow, Information object flow, Information flow computed by \alg.\\
    
    % $\muD^o_{uv}$ & Information object flow Decomposition \\
    % $\muD_{uv}$ & Information object flow Decomposition \\
    
    $\underline{\Emb}=[\Emb^{1}, \Emb^{2}, \ldots, \Emb^{\nCp}]$ & Chosen embedding for service collection $\mathcal R^T$.\\

    % $\mathcal I^{d,T}$ & Set of destination function of $\mathcal R^T$\\
    $\mathcal I^{d,T,\phi}; \mathcal K^{s,T,\phi}$ & Set of destination function of $\mathcal R^{T,\phi}$; Set of source functions of $\mathcal R^{T,\phi}$.\\
        
    \hline
    \end{tabular}
    \caption{Table summarizing main notation.}
    \label{tab:notations}
\end{table*}

